A methodology to evaluate continuum-scale yield surfaces based on the spatial distributions of yielding at the crystal scale

Using a correlation between local yielding and a multiaxial strength-to-stiffness parameter, the continuum-scale yield surface for a polyphase, polycrystalline solid is predicted. The predicted surface explicitly accounts for microstructure through the quantification of strength-to-stiffness based on a finite element model of a crystal-scale sample. The multiaxial strength-to-stiffness is evaluated from the elastic response of the sample and the restricted slip, single-crystal yield surface. Macroscopic yielding is defined by the propogation of a yield band through the sample and is detected with the aid of a flood fill agorithm. The methodology is demonstrated with the evaluation of a plane-stress yield surface for a dual-phase superaustenitic stainless steel.

==> piecewise.tex <==

Piecewise surfaces in either stress or deformation rate space
offer alternatives to analytical expansions for representing 
anisotropic strength.
A surface in stress space gives the anisotropic strength
directly via its shape.  
It also is possible to define a surface in deformation rate space
corresponding to a reference deformation rate.
The strength is represented as a field over the surface. 
Besides the strength, it is possible interpolate the stiffness 
over the surface, with the stiffness having been computed from 
polycrystal plasticity.
In this section we review two examples of piecewise representations
of strength.  The first is a surface in stress space and the second
a surface in deformation rate space over which the stiffness is interpolated.
\subsubsection{Hyperplane fits to the yield surface}
\label{sec:hyper_ys}
Maudlin and coworkers~\cite{mau_wri_gra_hou_95p,mau_wri_koc_sah_96}
have developed a methodology that utilizes a yield surface 
defined by hyperplanes in deviatoric stress space. 
The shape of the yield surface is defined by:
\beqn
 f_\chi \equiv \zeta_{ij}^\chi \sigma_{ij} - Y^\chi = 0, \chi = 1, 2, ..., m 
\label{eq:maudlin_ys}
\eeqn
and then scaled to the appropriate size according to:
\beqn
\sigma_{ij} = \tilde \sigma_{ij} {Y \over \bar M} 
\hspace{1cm}{\rm and} \hspace{1cm}
Y^\chi = {\tilde Y}^\chi  { Y \over \bar M}.
\eeqn
%{\bf  CHECK: Double check all the equations here.}
Here $\bar M$ is the average Taylor factor,
$Y^\chi$ is the minimum distance from the origin of
deviatoric stress space to the $\chi$ hyperplane, and
$\zeta_{ij}^\chi$ are the coefficients of the
normal vector to the $\chi$ hyperplane.  
The hyperplane data is determined by probing of 
the yield surface using crystal plasticity, together with the
measured ODF for a material, to find the yield strength
in a number of stress directions.  This set of points
is used in a tesselation algorithm to determine a
piecewise surface defined by Equation~\ref{eq:maudlin_ys}.   
Also needed is the flow law, which is obtained by
taking $f_\chi$ as a plastic potential and differentiating with
respect to the stress:
\beqn
\dot\epsilon^p_{ij} = 
\sum_{\chi = 1}^{m_{act}}  \dot\lambda^\chi \zeta_{ij}^\chi 
\label{eq:maudlin_fl}
\eeqn
where the linearity of $f_\chi$ with respect to $\sigma_{ij}$ has been 
exploited, $\dot\lambda^\chi$ are referred to as the loading scalars, and 
$m_{act}$ is the number of active hyperplanes, as explained below.

Maudlin and coworkers implemented the methodology 
in a formulation for dynamic analyses (an explicit formulation)   
and applied this approach to a number of applications.
While their applications have not been directed specifically at sheet forming,
the methodology generally is germane to the analysis of sheet.  
From an implementation perspective, 
the algorithm consists of 5 tasks that are performed for each time step.
For each step:
\begin{enumerate}
\item{determine if the stress at the beginning of the step satisfies
the equation of any of the hyperplanes (these are called admissible planes);}
\item{choose the most active candidate hyperplanes based on the
those having the largest loading scalars;}
\item{if so, determine if the material is being unloaded for any of the
admissible hyperplanes (those admissible planes that are not unloading
are called candidate planes);}
\item{using the candidate planes, determine the proportionality scalars 
from the consistency condition and back substitute into the hyperplane
equations to determine the stress;}
\item{perform a corrective step to reduce numerical errors.}
\end{enumerate}

The yield surface has been evaluated for clock-rolled zirconium plate.
The clock-rolled plate exhibited a strong basil texture aligned with plate
normal (ND) direction and an axisymmetric distribution about normal direction.
The degree of the resulting mechanical anisotropy is evident by 
the factor of four difference in the through-thickness and in-plane 
compressive strengths, as shown in Figure~\ref{fig:maudlin_ss}.
A partial representation of the surface is illustrated 
in Figure~\ref{fig:maudlin_ys}, which shows two projections 
of the surface onto three-dimensional subspaces.
The surfaces have been evaluated from the measured texture 
and a computation of the stresses corresponding to the nodes
of the tesselation.  There is a total of 203,125 nodes in the full
five-dimensional stress space representation based on a probe
interval of $15^\circ$ in the straining direction.  Only a small fraction
of the total set of nodes is shown in Figure~\ref{fig:maudlin_ys}.
The stress computations were performed using 
a viscoplastic self-consistent model~\cite{leb_tom_93,leb_tom_96} 
assuming a combination of prismatic and pyramidal slip 
systems~\cite{tom_mau_leb_kas_01}.
\subsubsection{Discretized flow anisotropic flow surface}
\label{sec:numer_ys}
Another alternative approach to the analytical description of the flow
surface given in Section~\ref{sec:analytic_ys} has been proposed by Durkot
and Dawson~\cite{daw_dur_01,durkot_ms} in which the stiffness is 
written as piecewise function over a reference deformation rate surface.
As presented in Section~\ref{sec:links_model},
the stresses can be calculated from the material stiffness and the
deformation rate, as given in Equation~\ref{eq:mstiff}. 
This equation defines a family of flow surfaces parameterized
by the deformation rate.  For a reference deformation rate magnitude,
${D}_{ref}$, the stiffness, $\mstiff_{ref}$, 
is evaluated for various deformation rate directions.  
Equation~\ref{eq:mstiff} then appears as:
\beqn
\label{eq:nodalstress}
\dkirch_{ref}=\mstiff_{ref} \pdefrate_{ref}
\eeqn
The reference deformation rate is scaled
to a magnitude appropriate for the applied deformation rate
as needed in a simulation.  
In general, the reference deformation rate defines a 
four dimensional surface within five dimensional deviatoric deformation
rate space.  It may be written in parametric form using piecewise interpolation
functions for both the deformation rate surface and the stiffness:
\beqn
\pdefrate_{ref} = \left[ N(\mb{\xi}) \right] 
\left\{ \pdefrate  \right\}
\label{eq:d_surf}
\eeqn
and
\beqn
\mstiff_{ref} = \left[ N(\mb{\xi})  \right] 
\left\{ \mstiff  \right\}
\label{eq:stiff_surf}
\eeqn
where 
$N(\mb{\xi})$ represents a set of continuous piecewise interpolation functions,
and $\mb{\xi}$ are local coordinates on a four dimensional surface used in the interpolation.
Linear interpolation was employed in \cite{durkot_ms}, 
but other interpolation functions are possible.  
Equations~\ref{eq:d_surf} and \ref{eq:stiff_surf} can be viewed as an
isoparametric finite element representation of the plastic stiffness.
It may also be convenient to store the stress over the deformation rate surface,
which may be done in the same manner using an isoparametric representation:
\beqn
\dkirch_{ref} = \left[ N(\mb{\xi}) \right] 
\left\{ \dkirch_j  \right\}
\eeqn
Equation~\ref{eq:nodalstress} is written for
deformation rates equal to the reference deformation rate.  In most 
problems, the deformation rates are not equal to the reference 
deformation rate  and scaling is required.
To scale the reference value of stiffness to the applied value, 
it was assumed that the behavior is viscoplastic and can be
described by a power law of the form (other forms are possible within the framework): 
\beqn
\label{eq:power-law}
\bar\tau = g \left(\frac{\bar{D}}{D_0}\right)^m 
\eeqn
where $g$ is a state variable proportional to the strength
~\cite{koc_76} and $\bar\tau$ and $\bar D$ appropriate scalar magnitudes  
of $\dkirch$ and $\pdefrate$, respectively.
For anisotropic response, the effective quantities are determined by requiring that 
the product of the effective stress and deformation rate yield the scalar plastic work rate , $\dot W$,
as shown below:  
\beqn
\dkirch=\lambda \: \hat{\mstiff} \: \pdefrate
\eeqn
where: 
\beqn
\lambda = c \left(\frac{\bar{\tau} }{\bar{D} } \right)
\eeqn
The parameter $\lambda$ is the magnitude of the stiffness, $\mstiff$, $c$ is a 
constant, and $\hat{\mstiff}$ is defined as:
\beqn
\hat{\mstiff} = \frac{\mstiff}{\lambda}
\eeqn
To ensure that: 
\beqn
\dot W = \dcauchy : \pdefrate = \pdefrate : \dcauchy
\eeqn
the effective quantities must be:
\beqn
{ \bar \sigma}  = \sqrt{c \: \dcauchy \hat{\mstiff} \dcauchy }
\hspace{1cm}
{\rm and} 
\hspace{1cm}
\label{eq:eff-d-aniso}
\bar{D}  = \sqrt{\frac{1}{c} \: \pdefrate \hat{\mstiff} \pdefrate}
\eeqn
The scaling then becomes: 
\beqn
\label{eq:final-scaling}
\mstiff=\mstiff_{ref} { \left( \frac {\bar D } {\bar{D}_{ref}}  \right)}^{m-1}
\eeqn

This construct of representing the flow surface has been evaluated 
for titanium sheet (Ti-6V-4Al) based on a combination of tensile
tests, measured texture, and a Taylor assumption computation 
(assuming prismatic, basal and pyramidal slip systems 
with strengths in the ratio of 1:1:5).
Figure~\ref{fig:durkot-0} shows a section of the yield surface for
a specimen whose tensile axis is aligned with the sheet rolling direction;
Figure~\ref{fig:durkot-90}  relates to specimen whose tensile axis
is perpendicular to the rolling direction.
If the material were isotropic, the stress vectors would be directed radially.
The presence of anisotropy is evident from the stress vectors being nearly parallel
in some regions and rapidly changing in others.
Notice that more concentrated points on the surface in stress space signifies 
more rapidly changing straining directions. 
By using a proper polycrystal representation to determine the material stiffnesses at each 
reference deformation rate point, there is a one-to-one correspondence between 
a stress and a deformation rate and normality is not violated.  In other 
words, this representation in deformation rate space produces an everywhere 
convex yield surface in stress space.  

%\input{Figures/maudlin1}
%\input{Figures/ti_sheet}


==> sx_yield_surface.tex <==
When loaded to a sufficient level, crystals deform plastically by slip on one or more slip systems. A slip system is active (meaning it contributes to the plastic straining of the crystal) if the resolved shear stress equals a critical value that depends on the its strength and the kinetics associated with dislocation motion. The collective consequence of the separate slip system constraints is to define the single crystal yield surface (SCYS). This is a closed surface in deviatoric stress space provided there is a sufficient number of independent slip systems. Further,  the associated slip modes span the five dimensional deviatoric deformation rate space, allowing the crystal to accommodate fully arbitrary isochoric plastic deformations. In the elastic stage of a loading process, the stress increases proportionally over a polycrystal, and eventually the favorably oriented crystals yield first, followed by ones with less favorable orientations. Both the directional strengths and stiffnesses of the crystals govern the order in which differently oriented crystals yield. The increasing stress levels within crystals are reflected in their lattice strains, which are elastic and can be monitored experimentally using x-ray diffraction. At yielding, the linearity associated with purely elastic response breaks down, and changes in the relative increases in lattice strains for differently oriented crystals are observed. This observation depends on the slip system strengths (SSS). The histories of the lattice strains as a sample is loaded beyond its initial yield stress and through its elastic-plastic transition thus provide an avenue to determine the relative slip system strengths. In this section,  the central points of the crystal mechanical behavior necessary to quantify slip system strengths from lattice strain data are discussed.    

\subsection{Yield surfaces for single crystals.}
\label{sec:scys}
In the modeling of the mechanical response of solids, yield surfaces dictate if and how a solid may deform plastically. For crystalline solids loaded at low to moderate temperature and moderate strain rates, the plastic deformation within a crystal often is dominated by crystallographic slip on a limited number of slip systems (commonly called restricted slip). Plastic flow by crystallographic slip is assumed to be isochoric and independent of the mean stress. It is also highly nonlinear and rate-dependent (viscoplastic). 

The yield surface for a single crystal (SCYS) is a combination of the separate relations for individual slip systems that each designate the stress required to activate slip on the system. For each slip system, $k$, the relation is that the magnitude of the resolved shear stress equals a critical value, where the resolved shear stress, $\rss$, is the projection of  the deviatoric crystal stress tensor, $\dcauchy$, onto the slip plane and into the slip direction \footnote{For ease of reading here, the relations are written in the current configuration without making distinctions between various configurations that arise in a kinematically nonlinear framework. Readers are referred to \cite{fepx} for more complete exposition.}. This  condition is simply stated using the symmetric portion of the Schmid tensor, $\symschmid$, as:
 \begin{equation}
\rss=\trace( \symschmid  \dcauchy) = \pm \tau^{\rm cr}
\label{eq:rss_projection}
\end{equation}
where the Schmid tensor for each slip system is defined by the diadic product of the slip plane normal, $\vctr{m}^k$, and slip direction, $\vctr{s}^k$. That is:
\begin{equation}
\symschmid  =  \mbox{\rm sym}(\schmid) \hspace{1cm}{\rm where }\hspace{1cm}  \schmid = \schmiddiad
\end{equation}
The critical value of the resolved shear stress, $\tau^{\rm cr}$, is rate dependent as a consequence of the kinetics of slip. The influence of the slip kinetics may be approximated mathematically over a modest range of strain rates using a power law expression between the resolved shear stress and the slip system shearing rate, $\gammadot$:
\begin{equation}
\tau^{\rm cr}=g^{k}({\frac{\| \gammadot \|}{\gdotz}})^m %\sign{\rss}
\label{eq:ss_kinetics}
\end{equation}
where $m$ is the rate sensitivity and $\gdotz$ is a scaling parameter. 
The critical resolved shear stress is scaled by the slip system strengths, $g^k$, which in general may be different for the various systems.

These relations collectively define a set of polytopes in deviatoric (five-dimensional) stress space, parameterized by the crystal plastic deformation rate, from the inner envelope of the set of planes given by Equation~\ref{eq:rss_projection}~\cite{lutjering_titanium_2007, rit_daw_mar_10}. If the crystal stress lies on a face of the yield surface, the crystal is plastically deforming via slip on the slip system associated with that face. For polyslip (plastic deformation involving multiple slip systems), the stress lies on an edge at the intersection of two faces or in a vertex created by the intersections of two or more edges. The deviatoric crystal plastic deformation rate is a linear combination of the slip system rates: 
\begin{equation}
{\tnsr{d}^p}^\prime =  \sumss \gammadot \symschmid
\label{eq:plasdefrate}
\end{equation}
where the symmetric portion of the Schmid tensor defines the simple shear deformation mode associated with deformation by slip for each system. 

The focus of this article is on yielding in HCP crystals, and in particular on the HCP, or $\alpha$, phase of  \TiSixFour. Section~\ref{sec:material} provides a description of the material and its initial mechanical state for {\it in situ} loading HEXD measurements. The volume fraction of the $\alpha$ phase is nominally 92\%. This phase dominates the mechanical behavior and, consequently, its properties are of greater interest. Three families of slip systems for the $\alpha$ phase are considered.  Because of the concentration of aluminum,  twinning is discounted as a possible deformation mode. The three slip system families are the basal, prismatic and pyramidal --  designations that reflect their orientations within the unit cell. Figure~\ref{tab:slipsystems} shows the slip system planes; Table~\ref{tab:slipsystems} lists the corresponding slip directions. 
Strengths of the basal, prismatic and pyramidal slip systems are designated as $g^b$, $g^p$ and $g^\pi$, respectively.
The combination of the three families generates a set of deformation modes that fully span the five-dimensional deviatoric deformation space and assures that the yield surface is closed.  
\begin{figure*}[ht!]
\label{fig:slipsystems}
    \centering
    \includegraphics[width=0.75\textwidth]{figure_1-hcp_ss.jpg}
    \caption{Primary slip systems for HCP phase of titanium. The slip plane normal is designated by $\vctr{m}$ and the slip direction is designated by $\vctr{s}$.}
\end{figure*}
\medskip
\begin{table}[ht]
\small
\centering
\begin{tabular}{|| c| c| c| c||}
\hline
 {\bf Slip System Name}	    	& {\bf Number of Systems}	& {\bf m}	& {\bf s}	\\
\hline
Basal (b)   	  & 3			& \hkl{0 0 0 1}	 & \hkl<1 1 -2 0>	\\
Prismatic (p)	  & 3			& \hkl{0 0 -1 0} & \hkl<1 1 -2 0>	\\
Pyramidal ($\pi$) & 12			& \hkl{0 0 -1 1}	& \hkl<1 1 -2 3>	\\
\hline
\end{tabular}
\caption{Slip systems for $\alpha$ phases.}
\label{tab:slipsystems}
\end{table}


\subsection{Elastic-plastic transition; role of strength-to-stiffness}
\label{sec:Y2E}
In polycrystals, grain interactions that arise as a consequence of the crystals simultaneously obeying the equations of kinematics and equilibrium affect the sequence of yielding among nearby crystals. The strength and the stiffness together regulate how the stresses in individual crystals reach the SCYS and activate slip~\cite{wong_influence_2010}. Thus, to use data that map the history of lattice strains through the elastic-plastic transition to quantify strength, it is necessary to account for the orientation dependence, or anisotropy, of the both the plastic and elastic behaviors.   For  elastic deformation,  the appropriate fixed-state relation for the mechanical response is simply Hooke's law, written using the stress-free configuration as a reference volume:
\begin{equation}
\kirch = \cofr \lateps 
\label{eq:hookes_law}
\end{equation}
where the Kirchhoff stress, $\kirch$, is written in the stress-free configuration as:
\begin{equation}
\kirch = \beta \cauchy  
\hspace{0.5 cm} {\rm where} \hspace{0.5cm} 
\beta = \detop (\latstretch) 
\label{eq:kirchhoff_defn}
\end{equation}
The elastic moduli for the \TiSixFour\, alloy studied here were evaluated previously using a combination of { \it in situ } loading HEXD data and finite element simulations\cite{wie_etal_2017}.   Optimized moduli were determined by minimizing an error defined by the square of the differences between the discrete harmonic coefficients for the experimental and  simulation lattice strains pole distributions.   These moduli are listed in
Table~\ref{tab:moduli}, along with a reference set for titanium for comparison, and were used in the simulations presented here.

The ratio of the directional strength to the directional modulus defines a parameter that is helpful in interpreting lattice strain trends in light of the relative strengths of slip systems. This parameter gives a ranking of crystals by orientation in terms of the proximity of the stress to the SCYS for crystals undergoing like deformation. Crystals with low strength-to-stiffness are more likely to first reach the SCYS in a polycrystal. Strictly, this interpretation of the strength to stiffness is limited to an iso-strain deformation environment.  However, averages taken over crystals lying on a specified crystallographic fiber (and thus corresponding to a particular diffraction condition) have been shown to rather closely follow the trends of the iso-strain condition~\cite{wong_influence_2010} for other crystal types. 

To quantify the directional strength,  the ratio of the SSS to the magnitude of the applied stress sufficient to place the stress on the SCYS~\cite{hosford_mechanics_1993} is specified. More precisely, for uniaxial tension, it is the ratio of the SSS to the minimum axial stress component required to satisfy Equation~\ref{eq:rss_projection} for at least one slip system. 
For crystal types with multiple slip system families, such as the $\alpha$ phase of titanium, the strength of one family is chosen for the purpose of computing the directionality of strength, namely the basal family (all of the family strengths enter the computation to determine the stress necessary to initiate slip through Equation~\ref{eq:rss_projection}, but only one strength is used to compute the strength metric).
As the relative values of the SSS are of primary interest, 
 the SSS ratios are designated using ($\tilde{g}^b$:$\tilde{g}^p$:$\tilde{g}^\pi$) = ($1$: (${g^p}/{g^b}$) : (${g^\pi}/{g^b}$)).

The strength-to-stiffness parameter is plotted  over the fundamental region of Rodrigues space for hexagonal crystal symmetry\footnote{For aid in interpreting the distributions over Rodrigues space, the locations of several important crystallographic fibers are shown in Appendix A.} in Figure~\ref{fig:Y2E_generic} for  two sets of slip system strength ratios: ($\tilde{g}^b$:$\tilde{g}^p$:$\tilde{g}^\pi$) = (1:1:1) and ($\tilde{g}^b$:$\tilde{g}^p$:$\tilde{g}^\pi$) =  (1:1:3).
For  ($\tilde{g}^b$:$\tilde{g}^p$:$\tilde{g}^\pi$) =  (1:1:3)  crystals with their c-axis aligned with the loading axis exhibit high strength-to-stiffness, and thus are  expected to remain elastic after other crystals have yielded. In contrast, for ($\tilde{g}^b$:$\tilde{g}^p$:$\tilde{g}^\pi$) = (1:1:1) the strength-to-stiffness ratio for crystals with their c-axis aligned with the loading axis is low, indicating that those crystals are expected to yield first in a tensile test. Lattice strain data are examined later in terms of the strength-to-stiffness distributions for different slip system strength sets.
\medskip
\begin{table}[ht]
\centering
  \begin{tabular}{|| c | c |c |c | c| c | c ||}
  \hline
  \hline
  Case & $C_{11}$ & $C_{12}$ & $C_{13}$ & $C_{44}$ & $\frac{E_{\rm max}}{E_{\rm min}}$ & $\frac{G_{\rm max}}{G_{\rm min}}$  \\ [0.5ex]
  \hline
  \hline
  \TiSixFour 	& 169 & 89 & 62 & 43 & 1.494  & 1.399   \\
  \hline
  Reference\cite{Kelly70} &161 & 91 &70 & 47 & 1.360 & 1.367\\
  \hline
  \hline
  \end{tabular}
\caption{\TiSixFour\, and reference single crystal elastic moduli (GPa)}
\label{tab:moduli}
\end{table}
\medskip
\begin{figure}[ht!]
\centering
    \includegraphics[width=1.0\textwidth]{figure_2-y2e_1to1to1+3.pdf}
\caption{Strength-to-stiffness ratio distributions for SSS ratios of (a) ($\tilde{g}^b$:$\tilde{g}^p$:$\tilde{g}^\pi$) = (1:1:1) and (b) ($\tilde{g}^b$:$\tilde{g}^p$:$\tilde{g}^\pi$) = (1:1:3) displayed over the fundamental region of Rodrigues space for HCP crystal symmetry. }
\label{fig:Y2E_generic}
\end{figure}
\newpage
